Stein $\Pi$-Importance Sampling

Stein discrepancies have emerged as a powerful tool for retrospective improvement of Markov chain Monte Carlo output. However, the question of how to design Markov chains that are well-suited to such post-processing has yet to be addressed. This paper studies Stein importance sampling, in which weights are assigned to the states visited by a $\Pi$-invariant Markov chain to obtain a consistent approximation of $P$, the intended target. Surprisingly, the optimal choice of $\Pi$ is not identical to the target $P$; we therefore propose an explicit construction for $\Pi$ based on a novel variational argument. Explicit conditions for convergence of Stein $\Pi$-Importance Sampling are established. For $\approx 70\%$ of tasks in the PosteriorDB benchmark, a significant improvement over the analogous post-processing of $P$-invariant Markov chains is reported.

==> inputs/full_results/posteriordb_plots.tex <==
\begin{figure}[!h]
    \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/toy_standard_normal_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/toy_mvsn_2d_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/earnings-earn_height_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/gp_pois_regr-gp_regr_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq-kidscore_momhs_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq-kidscore_momiq_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-logmesquite_logvolume_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/arma-arma11_KSDCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/earnings-logearn_logheight_male_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/garch-garch11_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq-kidscore_momhsiq_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/earnings-logearn_interaction_z_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq-kidscore_interaction_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq_with_mom_work-kidscore_interaction_c_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq_with_mom_work-kidscore_interaction_c2_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq_with_mom_work-kidscore_interaction_z_KSDCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/kidiq_with_mom_work-kidscore_mom_work_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/low_dim_gauss_mix-low_dim_gauss_mix_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-logmesquite_logva_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/hmm_example-hmm_example_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/sblrc-blr_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/sblri-blr_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/arK-arK_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-logmesquite_logvash_KSDCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/bball_drive_event_0-hmm_drive_0_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/bball_drive_event_1-hmm_drive_1_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/hudson_lynx_hare-lotka_volterra_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-logmesquite_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-logmesquite_logvas_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mesquite-mesquite_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/eight_schools-eight_schools_centered_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/eight_schools-eight_schools_noncentered_KSDCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1972-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1976-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1980-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1984-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1988-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1992-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes1996-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/nes2000-nes_KSDCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/diamonds-diamonds_KSDCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/full_results/mcycle_gp-accel_gp_KSDCurve_weight.pdf}
    \end{subfigure}\caption{\textcolor{red}{Chris to Add Caption.}}
\end{figure}
\FloatBarrier

==> inputs/full_results/wasd_plot.tex <==
\begin{figure}[!h]
    \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/toy_standard_normal_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/toy_mvsn_2d_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/earnings-earn_height_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/gp_pois_regr-gp_regr_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq-kidscore_momhs_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq-kidscore_momiq_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-logmesquite_logvolume_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/arma-arma11_wassCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/earnings-logearn_logheight_male_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/garch-garch11_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq-kidscore_momhsiq_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/earnings-logearn_interaction_z_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq-kidscore_interaction_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq_with_mom_work-kidscore_interaction_c_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq_with_mom_work-kidscore_interaction_c2_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq_with_mom_work-kidscore_interaction_z_wassCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/kidiq_with_mom_work-kidscore_mom_work_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/low_dim_gauss_mix-low_dim_gauss_mix_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-logmesquite_logva_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/hmm_example-hmm_example_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/sblrc-blr_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/sblri-blr_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/arK-arK_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-logmesquite_logvash_wassCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/bball_drive_event_0-hmm_drive_0_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/bball_drive_event_1-hmm_drive_1_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/hudson_lynx_hare-lotka_volterra_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-logmesquite_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-logmesquite_logvas_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mesquite-mesquite_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/eight_schools-eight_schools_centered_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/eight_schools-eight_schools_noncentered_wassCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1972-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1976-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1980-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1984-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1988-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1992-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes1996-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/nes2000-nes_wassCurve_weight.pdf}
    \end{subfigure}
    \caption{\textcolor{red}{Chris to Add Caption.}}
    \end{figure}
    \FloatBarrier

    \clearpage

    \begin{figure}[!h]
        \centering

    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/diamonds-diamonds_wassCurve_weight.pdf}
    \end{subfigure}
    \begin{subfigure}[!h]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/wasd_results/mcycle_gp-accel_gp_wassCurve_weight.pdf}
    \end{subfigure}\caption{\textcolor{red}{Chris to Add Caption.}}
\end{figure}
\FloatBarrier

==> inputs/garch-garch11/garch-garch11_marginal_distribution.tex <==
\begin{figure}[htpb]
    \centering
    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_para0.pdf}
    \end{subfigure}
    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_para1.pdf}
    \end{subfigure}

    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_para2.pdf}
    \end{subfigure}
    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_para3.pdf}
    \end{subfigure}

    \caption{\textcolor{red}{Chris to add caption and make decision on whether to include this figure.}}
\end{figure}

==> inputs/garch-garch11/garch-garch11_wksd.tex <==
\begin{figure}[htpb]
    \centering
    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_weight_s2.pdf}
    \end{subfigure}
    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_weight_s3.pdf}
    \end{subfigure}

    \begin{subfigure}[htpb]{0.49\textwidth}
        \includegraphics[width = 1\textwidth]{figures/garch-garch11/garch-garch11_weight_s4.pdf}
    \end{subfigure}


    \caption{\textcolor{red}{Chris to add caption and make decision on whether to include this figure.}}
\end{figure}
